Tx-LLM: A Large Language Model for Therapeutics

Developing therapeutics is a lengthy and expensive process that requires the satisfaction of many different criteria, and AI models capable of expediting the process would be invaluable. However, the majority of current AI approaches address only a narrowly defined set of tasks, often circumscribed within a particular domain. To bridge this gap, we introduce Tx-LLM, a generalist large language model (LLM) fine-tuned from PaLM-2 which encodes knowledge about diverse therapeutic modalities. Tx-LLM is trained using a collection of 709 datasets that target 66 tasks spanning various stages of the drug discovery pipeline. Using a single set of weights, Tx-LLM simultaneously processes a wide variety of chemical or biological entities(small molecules, proteins, nucleic acids, cell lines, diseases) interleaved with free-text, allowing it to predict a broad range of associated properties, achieving competitive with state-of-the-art (SOTA) performance on 43 out of 66 tasks and exceeding SOTA on 22. Among these, Tx-LLM is particularly powerful and exceeds best-in-class performance on average for tasks combining molecular SMILES representations with text such as cell line names or disease names, likely due to context learned during pretraining. We observe evidence of positive transfer between tasks with diverse drug types (e.g.,tasks involving small molecules and tasks involving proteins), and we study the impact of model size, domain finetuning, and prompting strategies on performance. We believe Tx-LLM represents an important step towards LLMs encoding biochemical knowledge and could have a future role as an end-to-end tool across the drug discovery development pipeline.

==> tables/training_on_drug_only_admet.tex <==
\begin{table}[htbp]
\centering
\caption{\textbf{\ourmodel exhibits signs of positive transfer across datasets with diverse drug types.} Performance of \ourmodels finetuned on various datasets and evaluated on the ADMET benchmark group. "All datasets" indicates a \ourmodels model finetuned on all TDC datasets, "molecule datasets" indicates a \ourmodels model finetuned on datasets containing molecules (datasets involving other drug types such as proteins or nucleic acids are not included in training), and "ADMET datasets" indicates a \ourmodels model finetuned on datasets in the ADMET benchmark, which only contains molecules.}
\label{tab:drug_only_admet}
\centerline{
\begin{tabular}{lccccc}
\toprule
Dataset name & Metric & All datasets & Molecule datasets & ADMET datasets \\
\midrule
HIA Hou & AUROC & \textbf{0.942} & 0.928 & 0.915 \\ 
Pgp Broccatelli & AUROC & 0.909 & \textbf{0.917} & 0.852 \\ 
Bioavailability Ma & AUROC & 0.605 & 0.667 & \textbf{0.713} \\ 
BBB Martins & AUROC & 0.805 & \textbf{0.860} & 0.843 \\ 
CYP2D6 Veith & AUPRC & \textbf{0.605} & 0.522 & 0.418 \\ 
CYP3A4 Veith & AUPRC & \textbf{0.800} & 0.737 & 0.736 \\ 
CYP2C9 Veith & AUPRC & \textbf{0.750} & 0.698 & 0.609 \\ 
CYP2C9 Substrate CarbonMangels & AUPRC & 0.403 & \textbf{0.455} & 0.328 \\ 
CYP2D6 Substrate CarbonMangels & AUPRC & 0.643 & 0.670 & \textbf{0.683} \\ 
CYP3A4 Substrate CarbonMangels & AUROC & 0.637 & \textbf{0.740} & 0.683 \\ 
hERG & AUROC & \textbf{0.879} & 0.857 & 0.753 \\ 
AMES & AUROC & \textbf{0.785} & 0.726 & 0.672 \\ 
DILI & AUROC & \textbf{0.727} & 0.628 & 0.524 \\ 
Caco2 Wang & MAE & 0.621 & 0.578 & \textbf{0.555} \\ 
Lipophilicity AstraZeneca & MAE & \textbf{0.779} & 0.815 & 0.813 \\ 
Solubility AqSolDB & MAE & 0.931 & 0.989 & \textbf{0.929} \\ 
PPBR AZ & MAE & \textbf{11.138} & 11.394 & 11.441 \\ 
VDss Lombardo & Spearman & \textbf{0.497} & 0.338 & 0.412 \\ 
Half Life Obach & Spearman & \textbf{0.525} & 0.316 & 0.267 \\ 
Clearance Hepatocyte AZ & Spearman & 0.256 & 0.154 & \textbf{0.262} \\ 
Clearance Microsome AZ & Spearman & 0.385 & 0.354 & \textbf{0.519} \\ 
LD50 Zhu & MAE & 0.808 & 0.749 & \textbf{0.713} \\
\bottomrule
\end{tabular}
}
\end{table}
